Many Hands Make Light Work: Using Essay Traits to Automatically Score Essays

Most research in the area of automatic essay grading (AEG) is geared towards scoring the essay holistically while there has also been some work done on scoring individual essay traits. In this paper, we describe a way to score essays holistically using a multi-task learning (MTL) approach, where scoring the essay holistically is the primary task, and scoring the essay traits is the auxiliary task. We compare our results with a single-task learning (STL) approach, using both LSTMs and BiLSTMs. We also compare our results of the auxiliary task with such tasks done in other AEG systems. To find out which traits work best for different types of essays, we conduct ablation tests for each of the essay traits. We also report the runtime and number of training parameters for each system. We find that MTL-based BiLSTM system gives the best results for scoring the essay holistically, as well as performing well on scoring the essay traits.

==> Rough.tex <==
\newpage
\ 
\newpage
% \appendix
\section{Comments}

Use this area for rough work, and other comments. Please note the new submission length for AAAI 2021 submissions - \textbf{\textit{seven pages}} of content, and up to \textit{two pages} of references.

\subsection{Sandeep's Comments}

\begin{enumerate}
\item Replaced the trait performances table with the figure.
\item Added some information about NLP-BEA 2020 papers.
\item Added some references from NLP-BEA 2020 and IJCAI-PRICAI 2020 papers.
\end{enumerate}

List of things to do:

\begin{enumerate}
\item Change the necessary citations to citeauthor citeyear.
\item Add the overall score functions in the supplementary material.
\item Add the performance table (Table \ref{Traits Results Table}) to the supplementary material.
\item Add an ethics statement at the end of the paper.
\end{enumerate}

\subsection{Sriparna Saha's Questions, Comments and Suggestions}

\begin{enumerate}
\item 
\end{enumerate}

\subsection{Pushpak Bhattacharyya's Questions, Comments and Suggestions}

\begin{enumerate}
\item 
\end{enumerate}

\subsection{Colour Codes}

Please use the following text colors for inserting suggestions / questions, etc. in the text of the paper (i.e. the file Paper.tex):
\begin{enumerate}
\item \textcolor{red}{Rahul Kumar - red}
\item \textcolor{blue}{Sandeep Mathias - blue}
\item \textcolor{orange}{Sriparna Saha - orange}
\item \textcolor{purple}{Pushpak Bhattacharyya - purple}
\end{enumerate}

In this file, you need not worry about using colour codes. Use colour codes mainly for suggestions / comments in Paper.tex.
% \textcolor{blue}{Sandeep}
